Hierarchical Classification for Spoken Arabic Dialect Identification using Prosody: Case of Algerian Dialects

In daily communications, Arabs use local dialects which are hard to identify automatically using conventional classification methods. The dialect identification challenging task becomes more complicated when dealing with an under-resourced dialects belonging to a same county/region. In this paper, we start by analyzing statistically Algerian dialects in order to capture their specificities related to prosody information which are extracted at utterance level after a coarse-grained consonant/vowel segmentation. According to these analysis findings, we propose a Hierarchical classification approach for spoken Arabic algerian Dialect IDentification (HADID). It takes advantage from the fact that dialects have an inherent property of naturally structured into hierarchy. Within HADID, a top-down hierarchical classification is applied, in which we use Deep Neural Networks (DNNs) method to build a local classifier for every parent node into the hierarchy dialect structure. Our framework is implemented and evaluated on Algerian Arabic dialects corpus. Whereas, the hierarchy dialect structure is deduced from historic and linguistic knowledges. The results reveal that within {\HD}, the best classifier is DNNs compared to Support Vector Machine. In addition, compared with a baseline Flat classification system, our HADID gives an improvement of 63.5% in term of precision. Furthermore, overall results evidence the suitability of our prosody-based HADID for speaker independent dialect identification while requiring less than 6s test utterances.

==> input/glance.tex <==

\section{A Glance at Algerian Arabic Dialects}
\label{Aglance}

%\subsection{Algerian Arabic Dialect Geography/ Typology Algerian Arabic Dialect }

Algeria is a large country   administratively divided into $48$ departments.  Its first  official  language  is MSA,  however  Algerian sub-dialects are widely the predominant means of communication. Algerian Arabic is used to refer to dialect spoken in Algeria, known as Daridjah to its speakers.  Algerian dialect presents  a complex linguistic features  mainly due to both Arabization processes that led to the appropriation of the Arabic language by populations  Berber origin, and  the deep colonization. In fact, Arabic Algerian dialect is affected by other languages such as Turkish, French, Italian, and Spanish~\cite{LECLERC2012}.




%It  is spoken  by  many borrowed words.  There are quite distinct local variations of Arabic dialects in the various departments  of Algeria. 


%Geographically, the Arabic dialect can be divided into  Eastern (ma\v{s}riq\={\i})  and Western (ma\.{g}rib\={\i}) group. The Western group  is a complex linguistic area. 


 %This complexity is mainly due to the Arabization process, in all regions of North Africa, and that led to the appropriation of the Arabic language by populations  Berber origin.
 
 
  According to the Arabization process, dialectologists show that Algerian Arabic  dialects can be divided into two major groups:  Pre-Hil\={a}l\={\i} and Bedouin dialect. Both dialects are different  by  many linguistic features~\cite{marçais1960Algeria} ~\cite{caubet2000questionnaire}.  




Firstly,  Pre-Hil\={a}l\={\i} dialect is called  sedentary dialect. It is spoken in areas that are affected  by the expansion of Islam in the $7^{th}$ century.  At this time, the partially affected cities are: Tlemcen, Constantine, and their rural surroundings. The other cities have  preserved their mother tongue language (Berber). Mar{\c{c}}ais \cite{marçais1977esquisse} has divided Pre-Hil\={a}l\={\i} dialect   into two dialects:  village (mountain), and urban dialect.  

\begin{itemize}
	\item   Village dialect is located  between  Trara mountains and Mediterranean  sea. The central town  of this area  is Nedroma, which is located in the  northwestern corner of Algeria.  There is also a village dialect  located in the northeastern corner of Algeria: it is  between  Collo, Djidjelli, and  Mila. %in the eastern  of B\'{e}ja\"{i}a
	
	\item 	Urban dialect is located  in the  northern cites: Tlemcen, Cherchell, Dellys, Djidjelli, and Collo.
\end{itemize}
 
 
  
  % In some towns the urban dialect is completely Bedouin: Annaba, Mascara, Mazouna, Mostaganem,  and Oran.
\begin{figure*}[t]
	\centering
	\scalebox{0.8} {\input{classificationDia2.tex}}
	\caption{Hierarchy Structure for Algerian Dialects.}
	\label{class1}
\end{figure*}  



Secondly, Bedouin dialect is spoken in areas which are  influenced by the Arab immigration in the $11^{th}$ century~\cite{PalvaH1},~\cite{PEREIRA1}.  Mar{\c{c}}ais \cite{marçais1960Algeria} has divided  Bedouin dialect into five  distinct basic dialects:
 
 \begin{enumerate}
 	\item Bedouin dialect of eastern Constantine, which are  located in  the region of El Kala and Souf.   It is called 'Sulaymite' dialect because it is connected with Tunisian Bedouin dialects.  
 	
 	\item Bedouin dialect of central and western side of Oran. It is called Ma'qilian dialect because it is connected with Moroccan Bedouin dialects. It covers a part of the arrondissement of Tlemcen, Oran, Sidi Bel Abb\`{e}s, and Sa\"{i}da. 
 	
 	
 	\item  Bedouin dialect of the Algerian central and of Sahara. It is  called Saharan Nomadic, it covers almost  the totality of the sahara of Algeria,  towards the east to Oued Righ,  towards the south to the Tadema\"{i}t plateau, and until the west (its limit has not  been clarified).  
 
 
 	\item Bedouin dialect of the Tell and of the Algerian-Oran Sahel. It is called Tellian Nomadic, that occupies a large part of the Tell of Algeria: Bordj Bou Arr\'{e}ridj, S\'{e}tif, El-Eulma, and El Kantara. 
 
 \item  The dialect of the high plains of Constantine, which covers  the north of Hodna region, and extends to the rough area from Bordj Bou Arr\'{e}ridj to Seybouse river.
 

 \end{enumerate}
 
 
 
 
  Mar{\c{c}}ais \cite{marçais1960Algeria} gathered   the  three dialects (3, 4, 5) under the name of  Hil\={a}l\={\i} dialect, which  takes its  name from  Ban\={u} Hil\={a}l tribe. In addition to that, there is  another dialect which has  urban dialects that have been completely influenced   by Bedouin dialect: Annaba, Algiers, B\'{e}ja\"{i}a, Blida,  Mascara, Mazouna, Mostaganem, Medea,   Mila,  Miliana,  Skikda, Tenes, and Oran. For that, we have classified these dialects, so-called  Urban Completely Bedouin (UCB), into the Bedouin dialects group.
  
  
  In spite of the sparse and the specific  linguistic  studies that have  dealt with  Arabic dialects, there is no efficient and complete  dialect hierarchy dedicated to Algerian dialects. We have  compiled a preliminary version of such  hierarchy from the above historical knowledges.  We summarize the Hierarchy structure for Algerian dialects  in Figure~\ref{class1}. This Hierarchy structure is also confirmed by some linguistic studies essentially   phonological, lexical and  morphological \cite{marçais1960Algeria} \cite{PalvaH12Classfi06}.  However, this Hierarchy structure has not benefited of deep prosodic analysis for that reason, in what follows, we study which prosodic features are discriminative for Algerian Arabic dialects. % These features are selected by  using statistic analysis  (One-way ANOVA).   %However, this classification has not beneficed of deep prosodic analysis.
 
  %In our study, we use this hierarchical structure  of Algerian dialects to perform our proposed {\HD} system. 
 
 

 
 %According to a historical classification used in Arabic dialectology

%\subsection{The Phonological Bases  of Algerian dialects}
%\label{sect:phoneticAlg}

%The classification of Arabic dialects into distinct geographical areas
%Geographical  Arabic dialects, the classification is essentially based on linguistic criteria: phonological, lexical and  morphological. We review the phonetic and phonological data  of Algerian Arabic dialects.

%Embarki \cite{embarki2008dialectes} resumes the descriptions proposed in the different bibliographic source, to identify the 'major'  discriminating phonological units for different types of  Arabic dialects.  He based mainly on the presence or absence of some phonemes of MSA in  Arabic dialects, this phonemes are four consonants: the dentals fricative \emph{/t, \underline{d}, \d{\underline{d}}/} and a voiceless uvular stop \emph{/q/}. For Algerian dialects classification, Versteegh  et al.  \cite{versteegh2006encyclopedia} used this four consonants  to discriminative the two major groups: Pre-Hil\={a}l\={\i} and Bedouin dialect, where Pre-Hil\={a}l\={\i} dialect   characterized by: \emph{/q/} is pronounced \emph{/k/} and the loss of inter-dentals  and pass into the dentals   \emph{/t, d, \d{d}/}. For Algerian Bedouin dialect, the four discriminative consonants are characterized by: /q/ is pronounced /g/ and  the inter-dentals are fairly preserved. 
%
%
%In addition,  Mar{\c{c}}ais \cite{marçais1960Algeria} presents  other  discriminative phonemes for two major  dialect groups  add the four discriminative features. For Pre-Hil\={a}l\={\i} dialect, the phonemes /k/ is pronounced as: a palatal [k\textsuperscript y], or an affricate [k\textsuperscript \textesh, t\textsuperscript \textesh], or as a fricative [\textesh]; /t/ is pronounced as an affricate [t\textsuperscript s]; /j/ becomes  [\textyogh] when it is single, and [d\textyogh] when it is doubled; the diphthongs /ay/ and /aw/ usually  become /{\=\i}/ and /\={u}/; /m/, /b/, /k/ have the ability to assimilate the article.
%
%The Bedouin  dialect characterized by  the preservation of diphthongs /ey/ and /ow/  or their  contraction  /{\=e}/ and /\={o}/. Each group have other dialect features  added   to the four discriminative consonants, which are presented in Table~\ref{table_hilalienPhon}.


%\begin{table}[h]
%	\centering
%	%\footnotesize
%	\input{Table/hilalienphonetic.tex}
%	\caption{Discriminative Consonants of Bedouin Dialects.}
%	\label{table_hilalienPhon}
%\end{table}


